Optimal Fairness Scheduling for Coded Caching in Multi-AP Wireless Local Area Networks

Coded caching (CC) schemes exploit the cumulative cache memory of the users and simple linear coding to turn unicast traffic (individual file requests) into a multicast transmission. For the originally proposed $K$-user single-server/single shared link network model, CC yields an $O(K)$ gain with respect to conventional uncoded caching with the same per-user memory. While several information-theoretic optimality results for a variety of problems and carefully crafted network topologies have been proved, the gains and suitability of CC for practical scenarios such as content streaming over existing wireless networks have not yet been fully demonstrated. In this work, we consider CC for on-demand video streaming over WLANs where multiple users are served simultaneously by multiple spatially distributed access points (AP). Users sequentially request video ``chunks". The CC scheme operates above the IP layer, leaving the underlying standard physical layer and MAC layer untouched. The cache placement is completely asynchronous and decentralized, and the users are placed at random over the network coverage area. For such a system, we consider the region of achievable long-term average delivery rate (defined as the number of video chunks delivered per unit of time) and study the per-user rate distribution under proportional fairness scheduling. We also consider reduced complexity scheduling strategies and compare them with standard state-of-the-art techniques such as conventional (uncoded) caching and collision avoidance by allocating APs on different sub-channels (i.e., frequency reuse).

==> Figs/CDF_Data_L.tex <==
Opt-L1-X	Opt-L1-Y	Super-L1-X	Super-L1-Y	Heur-L1-X	Heur-L1-Y	Opt-L5-X	Opt-L5-Y	Super-L5-X	Super-L5-Y	Heur-L5-X	Heur-L5-Y	Opt-L10-X	Opt-L10-Y	Super-L10-X	Super-L10-Y	Heur-L10-X	Heur-L10-Y	Opt-L15-X	Opt-L15-Y	Super-L15-X	Super-L15-Y	Heur-L15-X	Heur-L15-Y	Opt-L20-X	Opt-L20-Y
0.036202772	0	0.007513198	0	0.022616248	0	0.028945235	0	0.008220415	0	0.020861148	0	0.022778431	0	0.010573412	0	0.022963987	0	0.015174436	0	0.008440983	0	0.017298854	0	0.014509567	0
0.038155682	0.009259259	0.009474058	0.009259259	0.029401122	0.009259259	0.035976153	0.009259259	0.018755072	0.009259259	0.027513344	0.009259259	0.032896052	0.009259259	0.015236394	0.009259259	0.031199517	0.009259259	0.025564345	0.00778412	0.01452234	0.009191176	0.028725346	0.009191176	0.024930035	0.00778412
0.046319477	0.018518519	0.011680537	0.018518519	0.031662747	0.018518519	0.041837494	0.018518519	0.020088019	0.018518519	0.030720079	0.02037037	0.034771907	0.018518519	0.024331503	0.018518519	0.033592619	0.018518519	0.032008892	0.015568241	0.023402092	0.018382353	0.034548084	0.018382353	0.02942739	0.015568241
0.051861869	0.027777778	0.015083325	0.027777778	0.032206633	0.027777778	0.046856447	0.027777778	0.021944472	0.027777778	0.035675859	0.02962963	0.036890159	0.027777778	0.027948925	0.027777778	0.036998782	0.027777778	0.036315025	0.023611832	0.025233928	0.027573529	0.040604998	0.027573529	0.034046282	0.023611832
0.053774624	0.037037037	0.016482101	0.037037037	0.034687185	0.037037037	0.051415344	0.037037037	0.025404723	0.037037037	0.039018107	0.040740741	0.043386101	0.037037037	0.031353174	0.037037037	0.042567657	0.037037037	0.041459036	0.031655423	0.027766925	0.038602941	0.046582815	0.036764706	0.039469704	0.031395952
0.058071667	0.046296296	0.01741064	0.05	0.03597561	0.051851852	0.055706348	0.046296296	0.027540951	0.048148148	0.04541638	0.05	0.05299682	0.046296296	0.035410014	0.046296296	0.045228136	0.046296296	0.045494392	0.039439543	0.032293107	0.047794118	0.050639566	0.045955882	0.044720481	0.039180073
0.062709922	0.055555556	0.017862594	0.059259259	0.037308673	0.061111111	0.058183359	0.055555556	0.032001273	0.059259259	0.04789272	0.061111111	0.057723219	0.055555556	0.039127121	0.057407407	0.046720988	0.055555556	0.048903087	0.047483134	0.035054564	0.056985294	0.051840375	0.056985294	0.047392002	0.046964193
0.065109566	0.064814815	0.020459255	0.068518519	0.038414634	0.075925926	0.060176163	0.064814815	0.033964635	0.07037037	0.050144484	0.072222222	0.06162391	0.064814815	0.043869818	0.066666667	0.048886294	0.064814815	0.051641854	0.055267255	0.044010159	0.066176471	0.054906232	0.066176471	0.051530737	0.055267255
0.065222609	0.074074074	0.025585865	0.07962963	0.03902439	0.087037037	0.062954912	0.074074074	0.041311426	0.07962963	0.052491063	0.081481481	0.064560608	0.075925926	0.047284756	0.077777778	0.050335089	0.074074074	0.054785832	0.063570317	0.047968056	0.075367647	0.056075776	0.075367647	0.054540451	0.063310846
0.065222609	0.085185185	0.027952078	0.094444444	0.039859694	0.096296296	0.064086568	0.083333333	0.04321903	0.090740741	0.055495781	0.094444444	0.068410338	0.085185185	0.04990292	0.088888889	0.052272511	0.083333333	0.058056349	0.071873378	0.049886833	0.086397059	0.058574751	0.084558824	0.057246546	0.071873378
0.065222609	0.096296296	0.031271613	0.105555556	0.040322581	0.105555556	0.065060678	0.092592593	0.046765581	0.101851852	0.057458056	0.107407407	0.073286293	0.094444444	0.053109422	0.098148148	0.055618856	0.092592593	0.06336055	0.079916969	0.057825771	0.095588235	0.059768186	0.095588235	0.060002745	0.08017644
0.065827511	0.105555556	0.033974141	0.12037037	0.040778424	0.114814815	0.067286519	0.101851852	0.051289462	0.111111111	0.0598659	0.116666667	0.079194569	0.105555556	0.056531005	0.111111111	0.056470943	0.101851852	0.066171802	0.088479502	0.06062423	0.104779412	0.062448864	0.104779412	0.063149515	0.088220031
0.067821125	0.114814815	0.036770651	0.131481481	0.041624622	0.125925926	0.070228692	0.111111111	0.057152912	0.12037037	0.060999802	0.127777778	0.080845083	0.114814815	0.061155747	0.12037037	0.058123911	0.114814815	0.069400977	0.097301505	0.066442715	0.113970588	0.064353426	0.113970588	0.066904328	0.096263622
0.070062889	0.124074074	0.038198546	0.144444444	0.042729592	0.137037037	0.071906389	0.12037037	0.060299306	0.12962963	0.064977258	0.137037037	0.081323835	0.125925926	0.062679278	0.12962963	0.060660236	0.125925926	0.072410323	0.105345096	0.07321455	0.123161765	0.065279302	0.123161765	0.069113273	0.104566684
0.070786598	0.135185185	0.04050706	0.157407407	0.043197033	0.146296296	0.077081272	0.12962963	0.063965709	0.148148148	0.066292901	0.148148148	0.081818167	0.135185185	0.066593364	0.140740741	0.062414938	0.137037037	0.074077072	0.113129216	0.076734162	0.134191176	0.066584888	0.132352941	0.071946412	0.113129216
0.07250789	0.144444444	0.043736956	0.17037037	0.044412145	0.155555556	0.077208299	0.138888889	0.070620958	0.159259259	0.068226121	0.159259259	0.084558575	0.144444444	0.068859548	0.151851852	0.064849166	0.146296296	0.076288045	0.121432278	0.082052839	0.147058824	0.068514496	0.141544118	0.076573374	0.121172807
0.072507898	0.153703704	0.046121379	0.185185185	0.04509334	0.166666667	0.079389399	0.148148148	0.075469982	0.17962963	0.069692334	0.168518519	0.085042102	0.153703704	0.074143028	0.161111111	0.065535685	0.159259259	0.078328447	0.129216399	0.087176598	0.161764706	0.070659326	0.150735294	0.078491391	0.129216399
0.072507898	0.162962963	0.049204075	0.2	0.045968205	0.175925926	0.083694047	0.157407407	0.077710728	0.188888889	0.071247989	0.177777778	0.085701119	0.162962963	0.078081716	0.175925926	0.067765131	0.172222222	0.081427406	0.13751946	0.091982779	0.170955882	0.073132674	0.165441176	0.082241077	0.138557343
0.073473275	0.172222222	0.054542218	0.209259259	0.046644985	0.185185185	0.085452341	0.166666667	0.082585215	0.201851852	0.07239715	0.187037037	0.087084738	0.172222222	0.084202989	0.2	0.069580882	0.181481481	0.083392788	0.145563051	0.093522145	0.183823529	0.075068056	0.174632353	0.084855548	0.146600934
0.073567464	0.181481481	0.064407916	0.25	0.047305965	0.194444444	0.086361807	0.175925926	0.086763557	0.225925926	0.072902202	0.196296296	0.08908511	0.183333333	0.0859595	0.22037037	0.071453898	0.192592593	0.085054344	0.153347172	0.097793901	0.204044118	0.076855391	0.183823529	0.087944314	0.155163467
0.076920259	0.190740741	0.069585373	0.259259259	0.047642119	0.205555556	0.090072948	0.185185185	0.09044896	0.248148148	0.074664012	0.205555556	0.090207996	0.192592593	0.088292298	0.237037037	0.072947459	0.203703704	0.087281318	0.162169175	0.101448126	0.222426471	0.080460075	0.193014706	0.089953212	0.163466528
0.080789621	0.2	0.077218221	0.292592593	0.048356727	0.214814815	0.092280665	0.194444444	0.098092804	0.274074074	0.075661696	0.214814815	0.092264954	0.201851852	0.090402181	0.253703704	0.073567835	0.212962963	0.08933713	0.170212766	0.105168709	0.246323529	0.081867236	0.202205882	0.091796474	0.171510119
0.080789621	0.209259259	0.08565399	0.342592593	0.048909557	0.225925926	0.095417156	0.203703704	0.103801747	0.294444444	0.07710728	0.224074074	0.094537815	0.211111111	0.094537815	0.285185185	0.075172361	0.222222222	0.091662105	0.178256357	0.118183955	0.259191176	0.083284537	0.211397059	0.094278785	0.17929424
0.080789621	0.218518519	0.092358433	0.4	0.049320054	0.237037037	0.097739785	0.212962963	0.108323006	0.32037037	0.077863979	0.233333333	0.095083043	0.22037037	0.100298126	0.301851852	0.076488759	0.235185185	0.09414598	0.186559419	0.120796107	0.277573529	0.085621817	0.220588235	0.096189264	0.187597302
0.08138515	0.227777778	0.09761558	0.498148148	0.050063776	0.246296296	0.100833609	0.222222222	0.110959457	0.35	0.07851034	0.242592593	0.095450206	0.22962963	0.101777977	0.314814815	0.077365191	0.244444444	0.096673449	0.19460301	0.127742753	0.294117647	0.08718631	0.229779412	0.098878379	0.195900363
0.08138515	0.237037037	0.110888693	0.566666667	0.050496405	0.255555556	0.101750266	0.231481481	0.113850036	0.375925926	0.07931343	0.251851852	0.096689278	0.238888889	0.106668681	0.342592593	0.078270801	0.253703704	0.098702841	0.202646601	0.13067116	0.310661765	0.089048572	0.238970588	0.100774148	0.204203425
0.08243215	0.246296296	0.1182531	0.633333333	0.051679587	0.274074074	0.101850591	0.240740741	0.118827592	0.401851852	0.080341202	0.261111111	0.097824209	0.248148148	0.112899515	0.362962963	0.080019885	0.264814815	0.101097483	0.210430721	0.134110851	0.329044118	0.089619723	0.248161765	0.103290953	0.212506487
0.083333379	0.255555556	0.12471139	0.705555556	0.052083333	0.287037037	0.105136066	0.25	0.125553103	0.440740741	0.081347108	0.27037037	0.097848104	0.257407407	0.121959852	0.381481481	0.080749013	0.275925926	0.103494928	0.218474312	0.138996388	0.351102941	0.092201031	0.257352941	0.10705075	0.220550078
0.083333379	0.264814815	0.132912897	0.766666667	0.052890827	0.301851852	0.107990734	0.259259259	0.130372279	0.47037037	0.083314181	0.27962963	0.100672381	0.266666667	0.125247349	0.396296296	0.082282696	0.285185185	0.105190681	0.226258433	0.143089111	0.373161765	0.09358232	0.266544118	0.109562401	0.228593669
0.083333379	0.274074074	0.142630158	0.824074074	0.053607467	0.316666667	0.108222038	0.268518519	0.134704376	0.501851852	0.083861816	0.290740741	0.100672381	0.275925926	0.135444635	0.412962963	0.085166374	0.298148148	0.106787325	0.234302024	0.148441371	0.400735294	0.095654253	0.275735294	0.112116357	0.236377789
0.085282082	0.283333333	0.168489125	0.875925926	0.054432957	0.32962963	0.108483307	0.277777778	0.136680603	0.522222222	0.085007728	0.3	0.102552608	0.287037037	0.140468965	0.431481481	0.086022168	0.307407407	0.108488391	0.242345615	0.154335962	0.424632353	0.097948694	0.284926471	0.113227313	0.24416191
0.085282082	0.292592593	0.187247279	0.924074074	0.055216165	0.340740741	0.11151657	0.287037037	0.141352958	0.546296296	0.085976741	0.311111111	0.105793537	0.296296296	0.14299131	0.45	0.08691426	0.316666667	0.110334771	0.250129735	0.160686911	0.454044118	0.09894817	0.294117647	0.115137795	0.252205501
0.085850631	0.301851852	0.211254928	0.959259259	0.056125722	0.351851852	0.111665059	0.296296296	0.145708629	0.566666667	0.086685824	0.32037037	0.106502777	0.305555556	0.148102429	0.474074074	0.089901464	0.325925926	0.111715655	0.258692268	0.169122212	0.472426471	0.101371286	0.303308824	0.117649215	0.260768033
0.085850631	0.311111111	0.264788511	0.990740741	0.0566605	0.361111111	0.11191087	0.305555556	0.149664708	0.588888889	0.088013032	0.32962963	0.107236805	0.314814815	0.149994338	0.490740741	0.091458796	0.335185185	0.113526122	0.266476388	0.175675676	0.496323529	0.102215375	0.3125	0.119895978	0.269071095
0.085850819	0.32037037	0.264788511	0.990740741	0.057391524	0.372222222	0.112661685	0.314814815	0.153984887	0.607407407	0.089059986	0.338888889	0.108142257	0.324074074	0.153811234	0.507407407	0.092553253	0.344444444	0.115443751	0.274519979	0.188571572	0.509191176	0.103596664	0.321691176	0.122969078	0.276855215
0.088898534	0.32962963	0.264788511	0.990740741	0.057939092	0.381481481	0.113321516	0.324074074	0.166799504	0.625925926	0.089240184	0.35	0.111477997	0.333333333	0.15877005	0.527777778	0.094299131	0.353703704	0.118431385	0.2823041	0.199232121	0.522058824	0.10461187	0.330882353	0.126243412	0.284898806
0.089660749	0.338888889	0.264788511	0.990740741	0.05893186	0.390740741	0.114540625	0.333333333	0.170677353	0.644444444	0.089779529	0.362962963	0.114063702	0.342592593	0.16643834	0.548148148	0.096678387	0.364814815	0.12112926	0.290347691	0.225655633	0.540441176	0.106147097	0.340073529	0.128357879	0.292942398
0.089660749	0.348148148	0.264788511	0.990740741	0.059392265	0.4	0.114540628	0.342592593	0.17606288	0.661111111	0.090515043	0.372222222	0.114798033	0.351851852	0.169291363	0.566666667	0.098202043	0.374074074	0.122440781	0.298650752	0.228463006	0.566176471	0.107099062	0.349264706	0.129774329	0.301245459
0.091358797	0.357407407	0.264788511	0.990740741	0.060572687	0.411111111	0.115873219	0.351851852	0.179200783	0.677777778	0.091515497	0.383333333	0.116112985	0.361111111	0.173361559	0.587037037	0.09890247	0.385185185	0.124046794	0.306694344	0.233784087	0.590073529	0.108135504	0.358455882	0.131602696	0.309807992
0.091358797	0.366666667	0.264788511	0.990740741	0.06130064	0.422222222	0.117348897	0.361111111	0.183841334	0.696296296	0.09263981	0.392592593	0.118049797	0.37037037	0.17983606	0.607407407	0.101100393	0.394444444	0.126104201	0.314478464	0.246190079	0.610294118	0.11055387	0.369485294	0.133435455	0.318370524
0.095610733	0.375925926	0.264788511	0.990740741	0.062248611	0.431481481	0.118970187	0.37037037	0.195558419	0.724074074	0.093235469	0.401851852	0.121547027	0.37962963	0.189139025	0.627777778	0.102419384	0.403703704	0.127594396	0.322522055	0.250048543	0.630514706	0.112269818	0.380514706	0.134831042	0.326154645
0.095610733	0.385185185	0.264788511	0.990740741	0.063075506	0.440740741	0.121052186	0.37962963	0.203320964	0.740740741	0.094339623	0.411111111	0.121688502	0.388888889	0.204614036	0.638888889	0.105132048	0.412962963	0.129950614	0.330825117	0.258950877	0.648897059	0.114580769	0.389705882	0.136590094	0.334457706
0.096974846	0.394444444	0.264788511	0.990740741	0.06376241	0.45	0.121052996	0.388888889	0.209823963	0.757407407	0.095818815	0.422222222	0.12567598	0.398148148	0.227087143	0.65	0.105909014	0.424074074	0.131367462	0.338868708	0.264373532	0.685661765	0.118154449	0.398897059	0.137794063	0.342501297
0.096974846	0.403703704	0.264788511	0.990740741	0.06505102	0.459259259	0.121808987	0.398148148	0.218720749	0.77037037	0.09768985	0.433333333	0.126154025	0.409259259	0.241859344	0.666666667	0.108630579	0.433333333	0.133419468	0.346652828	0.266908675	0.707720588	0.121437957	0.408088235	0.139977762	0.350285418
0.097883869	0.412962963	0.264788511	0.990740741	0.065789474	0.47037037	0.12293803	0.407407407	0.223142536	0.8	0.098847416	0.442592593	0.126385531	0.418518519	0.244547306	0.67962963	0.109499623	0.444444444	0.136008552	0.35495589	0.277992776	0.731617647	0.123190845	0.419117647	0.142043721	0.358069538
0.097922636	0.422222222	0.264788511	0.990740741	0.067219153	0.47962963	0.123089936	0.416666667	0.229448962	0.814814815	0.099629791	0.451851852	0.130781042	0.42962963	0.258018221	0.696296296	0.111594128	0.455555556	0.137698125	0.362999481	0.284025134	0.753676471	0.124046372	0.428308824	0.143361725	0.365853659
0.097922636	0.431481481	0.264788511	0.990740741	0.069765649	0.490740741	0.123494351	0.425925926	0.249400347	0.82962963	0.101137318	0.462962963	0.135107877	0.438888889	0.267170583	0.709259259	0.114713891	0.47037037	0.140026097	0.370783601	0.293381703	0.777573529	0.127253282	0.439338235	0.144992504	0.373637779
0.098366548	0.440740741	0.264788511	0.990740741	0.071369344	0.501851852	0.124999966	0.435185185	0.263389049	0.842592593	0.101931027	0.472222222	0.137500355	0.448148148	0.274628391	0.722222222	0.116657056	0.47962963	0.141833339	0.378827193	0.296882742	0.805147059	0.128932464	0.448529412	0.146278802	0.382200311
0.098366548	0.451851852	0.264788511	0.990740741	0.072553897	0.512962963	0.125	0.444444444	0.282705917	0.853703704	0.103448276	0.481481481	0.140620076	0.457407407	0.279377614	0.735185185	0.117808195	0.488888889	0.142790857	0.386611313	0.304589742	0.841911765	0.130987577	0.457720588	0.147708866	0.390243902
0.102827377	0.461111111	0.264788511	0.990740741	0.073442312	0.525925926	0.125000001	0.453703704	0.315260563	0.862962963	0.105344505	0.492592593	0.14648899	0.466666667	0.282666641	0.748148148	0.118870161	0.498148148	0.144820645	0.395173845	0.31054516	0.863970588	0.136119453	0.470588235	0.149506829	0.398287494
0.104842598	0.47037037	0.264788511	0.990740741	0.075331971	0.537037037	0.125000009	0.462962963	0.328350166	0.875925926	0.106862072	0.505555556	0.148697755	0.475925926	0.292982475	0.766666667	0.122714575	0.507407407	0.145597157	0.402957966	0.315506126	0.887867647	0.139510174	0.479779412	0.151322979	0.406590555
0.104842598	0.47962963	0.264788511	0.990740741	0.076699834	0.548148148	0.126041979	0.472222222	0.33752285	0.888888889	0.107643525	0.514814815	0.149564219	0.485185185	0.298170058	0.785185185	0.123546252	0.516666667	0.147245354	0.410742086	0.335582102	0.915441176	0.141003293	0.488970588	0.15455642	0.414634146
0.106384056	0.488888889	0.264788511	0.990740741	0.078729282	0.559259259	0.126587917	0.481481481	0.356938359	0.901851852	0.109778242	0.527777778	0.151008572	0.494444444	0.304156568	0.803703704	0.126264949	0.525925926	0.14969168	0.419045148	0.351351351	0.950367647	0.143812197	0.498161765	0.156391264	0.422418267
0.106384056	0.498148148	0.264788511	0.990740741	0.079778704	0.57037037	0.127223055	0.490740741	0.363511829	0.914814815	0.112128287	0.537037037	0.153827387	0.503703704	0.308548604	0.82037037	0.129053128	0.537037037	0.15120885	0.426829268	0.363471417	0.972426471	0.147797907	0.516544118	0.158831629	0.430721328
0.108046314	0.507407407	0.264788511	0.990740741	0.081031308	0.57962963	0.129469496	0.5	0.387458029	0.927777778	0.114106122	0.548148148	0.156063828	0.512962963	0.319020684	0.833333333	0.130413983	0.546296296	0.152686938	0.434613389	0.483934319	0.998161765	0.149023296	0.525735294	0.160521324	0.43902439
0.108335949	0.516666667	0.264788511	0.990740741	0.082354443	0.588888889	0.132922294	0.509259259	0.40140499	0.937037037	0.115804972	0.557407407	0.158255984	0.522222222	0.327181198	0.859259259	0.133495758	0.557407407	0.15359951	0.442397509	0.483934319	0.998161765	0.150587787	0.551470588	0.161962478	0.447586923
0.109115983	0.525925926	0.264788511	0.990740741	0.08299285	0.598148148	0.133490073	0.518518519	0.417377148	0.95	0.116973619	0.566666667	0.160180828	0.531481481	0.332876681	0.875925926	0.134657119	0.566666667	0.154899875	0.450700571	0.483934319	0.998161765	0.153586217	0.560661765	0.166575262	0.456149455
0.109115983	0.535185185	0.264788511	0.990740741	0.08524335	0.607407407	0.135150749	0.527777778	0.431591469	0.961111111	0.118353248	0.575925926	0.164753064	0.540740741	0.338582726	0.890740741	0.136433009	0.575925926	0.156073757	0.458484691	0.483934319	0.998161765	0.157323118	0.569852941	0.1692763	0.463933576
0.110173926	0.544444444	0.264788511	0.990740741	0.086823289	0.618518519	0.135744419	0.537037037	0.446285073	0.97037037	0.119327222	0.585185185	0.170079343	0.55	0.341867014	0.924074074	0.138040295	0.585185185	0.156818147	0.466787753	0.483934319	0.998161765	0.161455899	0.579044118	0.174082074	0.472236637
0.110173926	0.553703704	0.264788511	0.990740741	0.089841539	0.62962963	0.137091583	0.546296296	0.453609331	0.97962963	0.12353482	0.594444444	0.171329594	0.559259259	0.347394401	0.938888889	0.139670403	0.594444444	0.158720196	0.474571873	0.483934319	0.998161765	0.163353438	0.608455882	0.177945929	0.480020758
0.110790484	0.562962963	0.264788511	0.990740741	0.092418546	0.638888889	0.143987646	0.555555556	0.498800694	0.990740741	0.126561382	0.603703704	0.17219705	0.568518519	0.359130655	0.966666667	0.142824287	0.609259259	0.160328997	0.482355994	0.483934319	0.998161765	0.169073393	0.619485294	0.182363755	0.488064349
0.111228693	0.572222222	0.264788511	0.990740741	0.09375	0.648148148	0.144216186	0.564814815	0.498800694	0.990740741	0.127556883	0.614814815	0.174013867	0.577777778	0.378151261	0.988888889	0.146280348	0.618518519	0.163045802	0.490659056	0.483934319	0.998161765	0.172942892	0.634191176	0.19102932	0.497405293
0.112180327	0.581481481	0.264788511	0.990740741	0.094476744	0.661111111	0.145540412	0.574074074	0.498800694	0.990740741	0.129438603	0.624074074	0.174169477	0.587037037	0.378151261	0.988888889	0.14812792	0.627777778	0.167270621	0.498443176	0.483934319	0.998161765	0.18163797	0.648897059	0.200067859	0.506227296
0.112612438	0.590740741	0.264788511	0.990740741	0.096619898	0.672222222	0.149739579	0.583333333	0.498800694	0.990740741	0.131680167	0.633333333	0.175520437	0.596296296	0.378151261	0.988888889	0.153082461	0.637037037	0.168242763	0.506486767	0.483934319	0.998161765	0.190736297	0.663602941	0.206254446	0.515827711
0.113215424	0.6	0.264788511	0.990740741	0.098214286	0.683333333	0.152720834	0.592592593	0.498800694	0.990740741	0.133017941	0.644444444	0.177003061	0.605555556	0.378151261	0.988888889	0.157354575	0.646296296	0.170347071	0.514270887	0.483934319	0.998161765	0.19546371	0.693014706	0.215381796	0.526984951
0.113215424	0.609259259	0.264788511	0.990740741	0.100316031	0.692592593	0.158456643	0.601851852	0.498800694	0.990740741	0.134246744	0.655555556	0.18794531	0.614814815	0.378151261	0.988888889	0.161814689	0.655555556	0.172708238	0.522055008	0.483934319	0.998161765	0.200286883	0.715073529	0.222441318	0.537882719
0.116031856	0.618518519	0.264788511	0.990740741	0.101513865	0.701851852	0.160115312	0.611111111	0.498800694	0.990740741	0.136249141	0.664814815	0.19183509	0.624074074	0.378151261	0.988888889	0.166612472	0.664814815	0.175975296	0.530098599	0.483934319	0.998161765	0.211892746	0.759191176	0.227099505	0.556305138
0.11793292	0.627777778	0.264788511	0.990740741	0.102209945	0.712962963	0.163598572	0.62037037	0.498800694	0.990740741	0.138861337	0.674074074	0.201388618	0.633333333	0.378151261	0.988888889	0.173376419	0.674074074	0.179206497	0.53814219	0.483934319	0.998161765	0.218541895	0.792279412	0.23291803	0.573430202
0.11793292	0.637037037	0.264788511	0.990740741	0.10469223	0.724074074	0.166347646	0.62962963	0.498800694	0.990740741	0.14032567	0.687037037	0.211255103	0.642592593	0.378151261	0.988888889	0.181326681	0.685185185	0.185067525	0.54592631	0.483934319	0.998161765	0.229783144	0.821691176	0.2386018	0.594187857
0.119601857	0.646296296	0.264788511	0.990740741	0.10626892	0.735185185	0.16666702	0.638888889	0.498800694	0.990740741	0.143324737	0.696296296	0.216559602	0.651851852	0.378151261	0.988888889	0.1895591	0.696296296	0.191270439	0.553710431	0.483934319	0.998161765	0.237686257	0.84375	0.246340444	0.616242865
0.119602873	0.655555556	0.264788511	0.990740741	0.107734807	0.744444444	0.167497588	0.648148148	0.498800694	0.990740741	0.147292204	0.705555556	0.222184232	0.661111111	0.378151261	0.988888889	0.194504973	0.705555556	0.195554782	0.561754022	0.483934319	0.998161765	0.245524093	0.875	0.254251561	0.640114167
0.119683561	0.664814815	0.264788511	0.990740741	0.11000283	0.753703704	0.170056834	0.657407407	0.498800694	0.990740741	0.152747471	0.714814815	0.230028172	0.67037037	0.378151261	0.988888889	0.197777335	0.714814815	0.203011644	0.570057084	0.483934319	0.998161765	0.256949961	0.90625	0.259642839	0.66787753
0.119683561	0.674074074	0.264788511	0.990740741	0.112799263	0.764814815	0.173013682	0.666666667	0.498800694	0.990740741	0.157621556	0.724074074	0.234730961	0.67962963	0.378151261	0.988888889	0.202631	0.731481481	0.21019055	0.578879087	0.483934319	0.998161765	0.28202132	0.948529412	0.266607846	0.697457187
0.120717259	0.683333333	0.264788511	0.990740741	0.118902439	0.774074074	0.178411794	0.675925926	0.498800694	0.990740741	0.168771777	0.733333333	0.240123343	0.692592593	0.378151261	0.988888889	0.208377778	0.746296296	0.216373134	0.58770109	0.483934319	0.998161765	0.319337128	0.976102941	0.271825877	0.727296316
0.127816992	0.692592593	0.264788511	0.990740741	0.122335271	0.783333333	0.180639902	0.685185185	0.498800694	0.990740741	0.173080738	0.742592593	0.24858812	0.701851852	0.378151261	0.988888889	0.215517906	0.766666667	0.223687951	0.596523093	0.483934319	0.998161765	0.333581257	0.998161765	0.277944248	0.757654385
0.127816992	0.701851852	0.264788511	0.990740741	0.123780488	0.792592593	0.190408766	0.694444444	0.498800694	0.990740741	0.175547879	0.751851852	0.260420751	0.711111111	0.378151261	0.988888889	0.224477881	0.787037037	0.232296401	0.607939803	0.483934319	0.998161765	0.333581257	0.998161765	0.284316737	0.791385573
0.127876513	0.711111111	0.264788511	0.990740741	0.130948305	0.801851852	0.190834311	0.703703704	0.498800694	0.990740741	0.178043791	0.762962963	0.273404346	0.731481481	0.378151261	0.988888889	0.230352214	0.801851852	0.238065757	0.624026985	0.483934319	0.998161765	0.333581257	0.998161765	0.290150929	0.821484172
0.128619568	0.72037037	0.264788511	0.990740741	0.133290816	0.811111111	0.193189822	0.712962963	0.498800694	0.990740741	0.181936322	0.772222222	0.284600914	0.744444444	0.378151261	0.988888889	0.237116333	0.818518519	0.246114259	0.640373638	0.483934319	0.998161765	0.333581257	0.998161765	0.296243467	0.857031655
0.131595403	0.72962963	0.264788511	0.990740741	0.13705446	0.82037037	0.194133822	0.722222222	0.498800694	0.990740741	0.184386973	0.781481481	0.29739551	0.77037037	0.378151261	0.988888889	0.24593963	0.846296296	0.252208401	0.65646082	0.483934319	0.998161765	0.333581257	0.998161765	0.303724619	0.887908666
0.132341908	0.738888889	0.264788511	0.990740741	0.140220735	0.82962963	0.194133822	0.731481481	0.498800694	0.990740741	0.188017557	0.790740741	0.302665021	0.787037037	0.378151261	0.988888889	0.257885578	0.864814815	0.260855719	0.680332122	0.483934319	0.998161765	0.333581257	0.998161765	0.315479884	0.918007265
0.132341908	0.748148148	0.264788511	0.990740741	0.142030034	0.838888889	0.195823797	0.740740741	0.498800694	0.990740741	0.193673922	0.801851852	0.308738605	0.805555556	0.378151261	0.988888889	0.263707553	0.896296296	0.268167655	0.703165542	0.483934319	0.998161765	0.333581257	0.998161765	0.324942508	0.945511157
0.140572519	0.757407407	0.264788511	0.990740741	0.142930503	0.848148148	0.203505659	0.75	0.498800694	0.990740741	0.198458133	0.811111111	0.315719752	0.82037037	0.378151261	0.988888889	0.267710658	0.916666667	0.275884467	0.723144785	0.483934319	0.998161765	0.333581257	0.998161765	0.350346064	0.973533991
0.141479954	0.768518519	0.264788511	0.990740741	0.144517822	0.857407407	0.207409983	0.759259259	0.498800694	0.990740741	0.203614983	0.82037037	0.320361655	0.838888889	0.378151261	0.988888889	0.273767735	0.935185185	0.281521494	0.751427089	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.14374257	0.77962963	0.264788511	0.990740741	0.147578204	0.866666667	0.214717731	0.768518519	0.498800694	0.990740741	0.208655332	0.82962963	0.32989634	0.855555556	0.378151261	0.988888889	0.282395847	0.955555556	0.289641291	0.784639336	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.14374257	0.788888889	0.264788511	0.990740741	0.156064914	0.875925926	0.218522538	0.777777778	0.498800694	0.990740741	0.21137965	0.838888889	0.342659189	0.885185185	0.378151261	0.988888889	0.308746226	0.985185185	0.295716961	0.809807992	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.143875899	0.798148148	0.264788511	0.990740741	0.168597561	0.885185185	0.218750018	0.787037037	0.498800694	0.990740741	0.215925449	0.848148148	0.348338954	0.907407407	0.378151261	0.988888889	0.368154306	1	0.303292449	0.83601453	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.148832377	0.807407407	0.264788511	0.990740741	0.172560976	0.894444444	0.220249234	0.796296296	0.498800694	0.990740741	0.225947109	0.857407407	0.352545528	0.925925926	0.378151261	0.988888889	0.368154306	1	0.30878319	0.861702128	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.148832377	0.816666667	0.264788511	0.990740741	0.178658537	0.903703704	0.22467691	0.805555556	0.498800694	0.990740741	0.238540692	0.866666667	0.364229713	0.953703704	0.378151261	0.988888889	0.368154306	1	0.31514279	0.88920602	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.148974724	0.825925926	0.264788511	0.990740741	0.187338501	0.912962963	0.230794157	0.814814815	0.498800694	0.990740741	0.243047575	0.877777778	0.377290247	0.977777778	0.378151261	0.988888889	0.368154306	1	0.324115062	0.915412558	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.149434582	0.835185185	0.264788511	0.990740741	0.198643411	0.922222222	0.239191248	0.824074074	0.498800694	0.990740741	0.252111761	0.887037037	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.337303403	0.938505449	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.153254996	0.844444444	0.264788511	0.990740741	0.2046716	0.931481481	0.254852782	0.833333333	0.498800694	0.990740741	0.259110539	0.9	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.351534789	0.964971458	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.156298575	0.853703704	0.264788511	0.990740741	0.219603763	0.940740741	0.270301497	0.842592593	0.498800694	0.990740741	0.272988506	0.914814815	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.389290752	0.985210171	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.156298575	0.862962963	0.264788511	0.990740741	0.232764748	0.95	0.294349632	0.853703704	0.498800694	0.990740741	0.290722997	0.925925926	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.694403385	1	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.168771848	0.872222222	0.264788511	0.990740741	0.261468675	0.959259259	0.314483897	0.864814815	0.498800694	0.990740741	0.304691484	0.938888889	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.694403385	1	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.170795357	0.881481481	0.264788511	0.990740741	0.297113752	0.968518519	0.331908986	0.877777778	0.498800694	0.990740741	0.317506676	0.95	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.694403385	1	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.171257102	0.890740741	0.264788511	0.990740741	0.323947278	0.977777778	0.339964546	0.887037037	0.498800694	0.990740741	0.337231969	0.962962963	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.694403385	1	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.172318139	0.9	0.264788511	0.990740741	0.39978678	0.987037037	0.376526935	0.898148148	0.498800694	0.990740741	0.360653723	0.977777778	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.694403385	1	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.1728954	0.909259259	0.264788511	0.990740741	0.424248228	0.996296296	0.387987403	0.912962963	0.498800694	0.990740741	0.381691479	0.988888889	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.694403385	1	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.181730204	0.918518519	0.264788511	0.990740741	0.424248228	0.996296296	0.395207587	0.927777778	0.498800694	0.990740741	0.434746328	0.998148148	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.694403385	1	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.207721204	0.927777778	0.264788511	0.990740741	0.424248228	0.996296296	0.406029958	0.940740741	0.498800694	0.990740741	0.434746328	0.998148148	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.694403385	1	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.208137307	0.937037037	0.264788511	0.990740741	0.424248228	0.996296296	0.416923053	0.95	0.498800694	0.990740741	0.434746328	0.998148148	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.694403385	1	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.213885096	0.946296296	0.264788511	0.990740741	0.424248228	0.996296296	0.434596453	0.961111111	0.498800694	0.990740741	0.434746328	0.998148148	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.694403385	1	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.226602479	0.957407407	0.264788511	0.990740741	0.424248228	0.996296296	0.44935382	0.972222222	0.498800694	0.990740741	0.434746328	0.998148148	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.694403385	1	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.252462932	0.966666667	0.264788511	0.990740741	0.424248228	0.996296296	0.463492874	0.981481481	0.498800694	0.990740741	0.434746328	0.998148148	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.694403385	1	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.276709096	0.975925926	0.264788511	0.990740741	0.424248228	0.996296296	0.509705564	0.994444444	0.498800694	0.990740741	0.434746328	0.998148148	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.694403385	1	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.285415811	0.985185185	0.264788511	0.990740741	0.424248228	0.996296296	0.509705564	0.994444444	0.498800694	0.990740741	0.434746328	0.998148148	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.694403385	1	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823
0.31732827	0.994444444	0.264788511	0.990740741	0.424248228	0.996296296	0.509705564	0.994444444	0.498800694	0.990740741	0.434746328	0.998148148	0.432080123	0.992592593	0.378151261	0.988888889	0.368154306	1	0.694403385	1	0.483934319	0.998161765	0.333581257	0.998161765	0.472872469	0.997145823

==> Figs/CDF_Data_U.tex <==
Opt-U10-X	Opt-U10-Y	Super-U10-X	Super-U10-Y	Heur-U10-X	Heur-U10-Y	Super-U20-X	Super-U20-Y	Heur-U20-X	Heur-U20-Y	Reuse-U20-X	Reuse-U20-Y	Reuse-U10-X	Reuse-U10-Y
0.00472425	0	0.001267256	0	0.003442222	0	0.000560484	0	0.001934012	0	0.003831418	0	0.006060606	0
0.005724487	0.006393862	0.001867657	0.006393862	0.003831858	0.006393862	0.000744556	0.003142678	0.002917068	0.006285355	0.003831418	0	0.006060606	0
0.007234356	0.012787724	0.002819482	0.012787724	0.004713185	0.012787724	0.000978149	0.006285355	0.003463803	0.01257071	0.003831418	0.004122423	0.006060606	0.004927386
0.007785554	0.019181586	0.003516759	0.019181586	0.005735239	0.019181586	0.001107636	0.009428033	0.003846781	0.019484601	0.003875969	0.007870081	0.006535948	0.022562241
0.008241216	0.025575448	0.00423945	0.025575448	0.006280656	0.025575448	0.001291521	0.013199246	0.004048843	0.025769956	0.004166667	0.019612742	0.006802721	0.03189834
0.008558123	0.031969309	0.004640288	0.035805627	0.006538939	0.031969309	0.001403774	0.016341923	0.004237979	0.032055311	0.004219409	0.027857589	0.007092199	0.040197095
0.008754928	0.038363171	0.005240156	0.042199488	0.007135444	0.038363171	0.001597921	0.019484601	0.004502944	0.038340666	0.004273504	0.031855091	0.007246377	0.047977178
0.009785905	0.044757033	0.005792324	0.04859335	0.007526309	0.046035806	0.001783847	0.022627278	0.004808025	0.045883092	0.004385965	0.039225484	0.007407407	0.051607884
0.010212901	0.051150895	0.006150093	0.056265985	0.0080457	0.052429668	0.001841452	0.025769956	0.005205656	0.052168448	0.004444444	0.050593379	0.007751938	0.059128631
0.010297687	0.057544757	0.006367858	0.063938619	0.008528785	0.060102302	0.00212162	0.028912634	0.005311046	0.059082338	0.004504505	0.058088695	0.007936508	0.070280083
0.010936444	0.063938619	0.006652888	0.070332481	0.008762179	0.066496164	0.002309083	0.032055311	0.005425143	0.065367693	0.00456621	0.069706433	0.008130081	0.092323651
0.011537531	0.070332481	0.006960016	0.076726343	0.009252555	0.072890026	0.002424896	0.035197989	0.005576723	0.07416719	0.004694836	0.076951905	0.008333333	0.123443983
0.011805829	0.076726343	0.007177832	0.083120205	0.009825122	0.08056266	0.002525566	0.038340666	0.005685968	0.080452546	0.004761905	0.083822611	0.008547009	0.141856846
0.012220477	0.083120205	0.007894489	0.090792839	0.010188978	0.086956522	0.002630021	0.041483344	0.005829421	0.086737901	0.004830918	0.087445347	0.00877193	0.174792531
0.012343228	0.089514066	0.00845083	0.097186701	0.010621095	0.094629156	0.002765391	0.045883092	0.00599238	0.093023256	0.004901961	0.097189257	0.009009009	0.209802905
0.01234403	0.095907928	0.008630871	0.106138107	0.01078561	0.101023018	0.003048741	0.04902577	0.006137532	0.100565682	0.004975124	0.110680824	0.009259259	0.226919087
0.012998808	0.10230179	0.009346945	0.112531969	0.011027504	0.10741688	0.003105488	0.053425519	0.006296086	0.106851037	0.005050505	0.130168645	0.00952381	0.262448133
0.013597405	0.108695652	0.009898281	0.118925831	0.011187222	0.113810742	0.003189707	0.056568196	0.006407256	0.115021999	0.005128205	0.146533417	0.009803922	0.310684647
0.013881435	0.115089514	0.01024326	0.125319693	0.01141671	0.120204604	0.003312426	0.060339409	0.006498279	0.121935889	0.005208333	0.165646471	0.01010101	0.351919087
0.013891632	0.121483376	0.011017783	0.131713555	0.011546445	0.126598465	0.003411921	0.063482087	0.00660744	0.130106851	0.005291005	0.19412867	0.010416667	0.374740664
0.014451345	0.127877238	0.011394564	0.145780051	0.011805916	0.132992327	0.003573964	0.067881835	0.006723558	0.137020742	0.005376344	0.227607745	0.010752688	0.41623444
0.015108229	0.1342711	0.011897314	0.153452685	0.012000519	0.140664962	0.00361019	0.071024513	0.006823692	0.143934632	0.005464481	0.250093691	0.011111111	0.476919087
0.016517276	0.140664962	0.01288969	0.16112532	0.012246886	0.148337596	0.003681969	0.07416719	0.006924883	0.150219987	0.005555556	0.283447845	0.011494253	0.524636929
0.016666666	0.147058824	0.013142728	0.167519182	0.012458737	0.15601023	0.003723968	0.077938404	0.007042254	0.157762414	0.005649718	0.297564022	0.011904762	0.558350622
0.016666667	0.153452685	0.013603244	0.181585678	0.012778192	0.162404092	0.003795009	0.082966688	0.007219759	0.164676304	0.005747126	0.330668332	0.012345679	0.617738589
0.016871326	0.159846547	0.014119109	0.18797954	0.012997305	0.168797954	0.003854347	0.086109365	0.007310924	0.171590195	0.005847953	0.363897564	0.012820513	0.668309129
0.017205688	0.166240409	0.014605288	0.194373402	0.01311449	0.175191816	0.004149686	0.089880578	0.00743349	0.17787555	0.005952381	0.40387258	0.013333333	0.691130705
0.017693163	0.172634271	0.015831561	0.200767263	0.013310617	0.181585678	0.004245164	0.093023256	0.007535014	0.185417976	0.006060606	0.445096814	0.013888889	0.729253112
0.01814497	0.179028133	0.016743355	0.207161125	0.013466502	0.18797954	0.004347683	0.096794469	0.00766241	0.191703331	0.00617284	0.487695191	0.014492754	0.786307054
0.01839348	0.185421995	0.017099233	0.21483376	0.013622211	0.195652174	0.004498614	0.099937146	0.00778974	0.197988686	0.006289308	0.509431605	0.015151515	0.800570539
0.018629656	0.191815857	0.017833023	0.226342711	0.013708162	0.203324808	0.004585664	0.10370836	0.007907425	0.206159648	0.006410256	0.534041224	0.015873016	0.853215768
0.018715088	0.198209719	0.018537313	0.24168798	0.014056036	0.20971867	0.004611633	0.108108108	0.00801956	0.21433061	0.006535948	0.569768894	0.016666667	0.882780083
0.019130352	0.204603581	0.019281054	0.260869565	0.014385667	0.217391304	0.004763852	0.111250786	0.008111174	0.2212445	0.006666667	0.593878826	0.01754386	0.908713693
0.019571812	0.210997442	0.019616626	0.280051151	0.014667168	0.223785166	0.004854637	0.114393463	0.008258355	0.228786926	0.006802721	0.622361024	0.018518519	0.929460581
0.019820163	0.217391304	0.020657398	0.296675192	0.01492723	0.230179028	0.005094197	0.117536141	0.008336216	0.235700817	0.006944444	0.659462836	0.019607843	0.96343361
0.02	0.223785166	0.021435982	0.305626598	0.015059961	0.23657289	0.005196525	0.121307354	0.008509651	0.242614708	0.007092199	0.708557152	0.020833333	0.966026971
0.020150517	0.230179028	0.021745226	0.320971867	0.015318146	0.242966752	0.005279467	0.124450031	0.008604718	0.248900063	0.007246377	0.742910681	0.022222222	0.969139004
0.020174466	0.23657289	0.022500001	0.337595908	0.015452245	0.250639386	0.00553518	0.127592709	0.008717379	0.257071025	0.007407407	0.772642099	0.023809524	0.98469917
0.020497435	0.242966752	0.023201554	0.355498721	0.015524423	0.257033248	0.005606777	0.131363922	0.008851744	0.263984915	0.007575758	0.805371643	0.025641026	0.991960581
0.020814265	0.249360614	0.023446285	0.372122762	0.015929204	0.264705882	0.005751551	0.135135135	0.008958838	0.270898806	0.007751938	0.835227983	0.03030303	0.993516598
0.020837449	0.255754476	0.024337047	0.386189258	0.016076696	0.271099744	0.005863588	0.138277813	0.009090909	0.277812696	0.007936508	0.851592755	0.033333333	0.998184647
0.021008261	0.262148338	0.024742446	0.404092072	0.016244028	0.277493606	0.006092999	0.142049026	0.009185149	0.285355123	0.008130081	0.87532792	0.037037037	0.998962656
0.021500431	0.268542199	0.025208969	0.423273657	0.016552575	0.28516624	0.006146187	0.145820239	0.009285342	0.292269013	0.008333333	0.890068707	0.047619048	1
0.021580787	0.274936061	0.025844199	0.442455243	0.016628783	0.291560102	0.006287403	0.149591452	0.0094392	0.299182904	0.008547009	0.902935665	0.047619048	1
0.021772032	0.281329923	0.02682782	0.455242967	0.016839468	0.297953964	0.006367746	0.152734129	0.009560097	0.305468259	0.00877193	0.925796377	0.047619048	1
0.022116453	0.287723785	0.027800137	0.469309463	0.016961652	0.304347826	0.006504983	0.156505343	0.009672237	0.31238215	0.009009009	0.938038726	0.047619048	1
0.022396889	0.294117647	0.028412113	0.488491049	0.017109145	0.31202046	0.006592508	0.160276556	0.009777621	0.31929604	0.009259259	0.948657089	0.047619048	1
0.022396892	0.300511509	0.029952603	0.498721228	0.017319998	0.319693095	0.006747456	0.164676304	0.009910581	0.327467002	0.00952381	0.955277951	0.047619048	1
0.022500004	0.306905371	0.030721188	0.523017903	0.017516984	0.326086957	0.006828113	0.169076053	0.010045029	0.333752357	0.009803922	0.962398501	0.047619048	1
0.022835287	0.313299233	0.031427679	0.542199488	0.0176586	0.332480818	0.007241311	0.17221873	0.010161022	0.340666248	0.01010101	0.975140537	0.047619048	1
0.02306256	0.319693095	0.032101494	0.554987212	0.01794191	0.340153453	0.007600331	0.175361408	0.01027001	0.347580138	0.010416667	0.976764522	0.047619048	1
0.023074981	0.326086957	0.033085943	0.569053708	0.018124178	0.346547315	0.007752936	0.178504085	0.01038312	0.355122564	0.010752688	0.98113679	0.047619048	1
0.023138617	0.332480818	0.033861039	0.588235294	0.018228592	0.352941176	0.007853811	0.181646763	0.010480802	0.363293526	0.011111111	0.982510931	0.047619048	1
0.023214296	0.33887468	0.034246779	0.603580563	0.018584071	0.359335038	0.008232567	0.185417976	0.010602504	0.370207417	0.011494253	0.991880075	0.047619048	1
0.023292499	0.345268542	0.034760768	0.615089514	0.018701367	0.367007673	0.008271814	0.189189189	0.010730674	0.377121307	0.011904762	0.994753279	0.047619048	1
0.023405588	0.351662404	0.035281432	0.627877238	0.018961598	0.373401535	0.008400658	0.193588938	0.010800386	0.387806411	0.012345679	0.997501562	0.047619048	1
0.02356368	0.358056266	0.03563557	0.645780051	0.019147372	0.379795396	0.008684738	0.197360151	0.010907825	0.395348837	0.012820513	0.998750781	0.047619048	1
0.024810005	0.364450128	0.036345432	0.659846547	0.019276445	0.386189258	0.008952177	0.205531113	0.010972701	0.403519799	0.013888889	1	0.047619048	1
0.024999966	0.37084399	0.036807666	0.672634271	0.019619113	0.39258312	0.009233862	0.20867379	0.011060692	0.409805154	0.013888889	1	0.047619048	1
0.025	0.377237852	0.038012248	0.685421995	0.01975087	0.400255754	0.009282256	0.211816468	0.011177347	0.416090509	0.013888889	1	0.047619048	1
0.025000011	0.383631714	0.038506294	0.696930946	0.020078936	0.406649616	0.009541401	0.214959145	0.011239288	0.4230044	0.013888889	1	0.047619048	1
0.025000083	0.390025575	0.03945266	0.71483376	0.020355711	0.413043478	0.009903698	0.228158391	0.011316527	0.42991829	0.013888889	1	0.047619048	1
0.025557421	0.396419437	0.040408273	0.730179028	0.020592526	0.420716113	0.010185818	0.231301069	0.011404087	0.438089252	0.013888889	1	0.047619048	1
0.025641646	0.402813299	0.042383724	0.74168798	0.020766937	0.427109974	0.010367554	0.234443746	0.011512605	0.444374607	0.013888889	1	0.047619048	1
0.025737219	0.409207161	0.043202043	0.757033248	0.021014543	0.433503836	0.010663498	0.245757385	0.011610194	0.450659962	0.013888889	1	0.047619048	1
0.026135717	0.415601023	0.044095877	0.771099744	0.021296986	0.441176471	0.010853989	0.259585167	0.011719026	0.456945317	0.013888889	1	0.047619048	1
0.02654568	0.421994885	0.044862855	0.782608696	0.021407235	0.447570332	0.011010345	0.262727844	0.011913511	0.465116279	0.013888889	1	0.047619048	1
0.026897517	0.428388747	0.046167647	0.799232737	0.021567351	0.453964194	0.011460354	0.277812696	0.012032932	0.473287241	0.013888889	1	0.047619048	1
0.027017447	0.434782609	0.047563539	0.81202046	0.02173913	0.460358056	0.01199703	0.294783155	0.012102243	0.479572596	0.013888889	1	0.047619048	1
0.027207408	0.441176471	0.049250556	0.822250639	0.02189781	0.468030691	0.012265541	0.303582652	0.012240896	0.486486486	0.013888889	1	0.047619048	1
0.027371922	0.447570332	0.05	0.833759591	0.022079861	0.474424552	0.012596432	0.320553111	0.012415622	0.493400377	0.013888889	1	0.047619048	1
0.027783264	0.453964194	0.051254051	0.841432225	0.022206131	0.482097187	0.012823455	0.33186675	0.012571727	0.500942803	0.013888889	1	0.047619048	1
0.028594169	0.460358056	0.053596891	0.847826087	0.022381477	0.488491049	0.012986231	0.344437461	0.012742176	0.507228158	0.013888889	1	0.047619048	1
0.02875003	0.466751918	0.057483982	0.854219949	0.022545404	0.496163683	0.013183566	0.355122564	0.012889029	0.514770585	0.013888889	1	0.047619048	1
0.028810548	0.47314578	0.059005321	0.861892583	0.022722918	0.502557545	0.013670963	0.362036455	0.013013517	0.52105594	0.013888889	1	0.047619048	1
0.029230252	0.479539642	0.062713554	0.869565217	0.023000745	0.508951407	0.013981685	0.373350094	0.013178831	0.527341295	0.013888889	1	0.047619048	1
0.029585099	0.485933504	0.065637533	0.879795396	0.023066711	0.515345269	0.01441385	0.388434947	0.01340405	0.534883721	0.013888889	1	0.047619048	1
0.029835954	0.492327366	0.06988952	0.886189258	0.023300048	0.52173913	0.014642956	0.39912005	0.013543599	0.542426147	0.013888889	1	0.047619048	1
0.030286123	0.498721228	0.071541383	0.893861893	0.023474792	0.528132992	0.015014939	0.41734758	0.013586397	0.549340038	0.013888889	1	0.047619048	1
0.030472016	0.50511509	0.073112815	0.901534527	0.023730501	0.534526854	0.015388367	0.433689503	0.013732394	0.556882464	0.013888889	1	0.047619048	1
0.030738149	0.511508951	0.074227337	0.907928389	0.02395911	0.542199488	0.015601892	0.446888749	0.013887531	0.56442489	0.013888889	1	0.047619048	1
0.030766642	0.517902813	0.076024495	0.914322251	0.02417208	0.54859335	0.015892986	0.458202388	0.014054966	0.571338781	0.013888889	1	0.047619048	1
0.030927062	0.524296675	0.077861223	0.925831202	0.024449196	0.554987212	0.016196289	0.470773099	0.014232489	0.578881207	0.013888889	1	0.047619048	1
0.031163027	0.530690537	0.07921361	0.932225064	0.025058082	0.561381074	0.016480122	0.48460088	0.014439519	0.587680704	0.013888889	1	0.047619048	1
0.031163027	0.537084399	0.080816546	0.941176471	0.025211319	0.567774936	0.016939138	0.49717159	0.014577425	0.593966059	0.013888889	1	0.047619048	1
0.03120745	0.543478261	0.082141128	0.952685422	0.025505329	0.574168798	0.017199967	0.512256442	0.014692844	0.600251414	0.013888889	1	0.047619048	1
0.031432268	0.549872123	0.084767448	0.959079284	0.025747823	0.58056266	0.017569391	0.526712759	0.014843548	0.606536769	0.013888889	1	0.047619048	1
0.031590215	0.556265985	0.088722072	0.969309463	0.025914782	0.586956522	0.017911786	0.539912005	0.014977645	0.61345066	0.013888889	1	0.047619048	1
0.032055269	0.562659847	0.090660332	0.97826087	0.026094953	0.593350384	0.018280659	0.552482715	0.01521377	0.619736015	0.013888889	1	0.047619048	1
0.032291256	0.569053708	0.096292807	0.985933504	0.026401413	0.599744246	0.01846104	0.565681961	0.015406162	0.627906977	0.013888889	1	0.047619048	1
0.032701205	0.57544757	0.1	0.998721228	0.026806817	0.60741688	0.018693812	0.5769956	0.015584833	0.635449403	0.013888889	1	0.047619048	1
0.03333302	0.581841432	0.1	0.998721228	0.027068402	0.616368286	0.019165745	0.588937775	0.01570773	0.642991829	0.013888889	1	0.047619048	1
0.033333333	0.588235294	0.1	0.998721228	0.027374451	0.622762148	0.019334144	0.598994343	0.015825298	0.64990572	0.013888889	1	0.047619048	1
0.033333333	0.594629156	0.1	0.998721228	0.027606329	0.630434783	0.019583166	0.608422376	0.015994398	0.65681961	0.013888889	1	0.047619048	1
0.033595334	0.601023018	0.1	0.998721228	0.027688981	0.636828645	0.020353339	0.619736015	0.016079812	0.665619107	0.013888889	1	0.047619048	1
0.033835993	0.60741688	0.1	0.998721228	0.028504096	0.643222506	0.020523616	0.627278441	0.01627543	0.672532998	0.013888889	1	0.047619048	1
0.033905506	0.613810742	0.1	0.998721228	0.028877601	0.649616368	0.02089096	0.637335009	0.016414566	0.680075424	0.013888889	1	0.047619048	1
0.034084328	0.620204604	0.1	0.998721228	0.029190295	0.65601023	0.021428515	0.646763042	0.016554889	0.686360779	0.013888889	1	0.047619048	1
0.034198306	0.626598465	0.1	0.998721228	0.029640197	0.662404092	0.021741211	0.655562539	0.016644693	0.692646135	0.013888889	1	0.047619048	1
0.034914462	0.632992327	0.1	0.998721228	0.030332287	0.668797954	0.021844117	0.667504714	0.016909621	0.699560025	0.013888889	1	0.047619048	1
0.035383776	0.639386189	0.1	0.998721228	0.031120944	0.676470588	0.022128587	0.676932747	0.017056758	0.707102451	0.013888889	1	0.047619048	1
0.035532512	0.645780051	0.1	0.998721228	0.03145223	0.68286445	0.022583615	0.688246386	0.017156693	0.713387806	0.013888889	1	0.047619048	1
0.035885159	0.652173913	0.1	0.998721228	0.031996015	0.689258312	0.022903345	0.69893149	0.017289424	0.719673162	0.013888889	1	0.047619048	1
0.036242831	0.658567775	0.1	0.998721228	0.03259587	0.695652174	0.023429635	0.70584538	0.017507942	0.726587052	0.013888889	1	0.047619048	1
0.036745823	0.664961637	0.1	0.998721228	0.033038348	0.705882353	0.023972111	0.715273413	0.01775503	0.732872407	0.013888889	1	0.047619048	1
0.036954652	0.671355499	0.1	0.998721228	0.033485393	0.71483376	0.024260531	0.724701446	0.017898458	0.739157762	0.013888889	1	0.047619048	1
0.038058811	0.677749361	0.1	0.998721228	0.033800301	0.721227621	0.02461229	0.732872407	0.018083008	0.747328724	0.013888889	1	0.047619048	1
0.03821816	0.684143223	0.1	0.998721228	0.033990659	0.727621483	0.024834054	0.744186047	0.018394407	0.754242615	0.013888889	1	0.047619048	1
0.038455982	0.690537084	0.1	0.998721228	0.034315245	0.734015345	0.024932769	0.754242615	0.018999367	0.76052797	0.013888889	1	0.047619048	1
0.038564361	0.696930946	0.1	0.998721228	0.034660767	0.74168798	0.025237404	0.763670647	0.019343452	0.768070396	0.013888889	1	0.047619048	1
0.039376941	0.703324808	0.1	0.998721228	0.035386045	0.748081841	0.025647278	0.771841609	0.019553599	0.776241358	0.013888889	1	0.047619048	1
0.039832382	0.70971867	0.1	0.998721228	0.035879511	0.754475703	0.025982217	0.783155248	0.019986145	0.782526713	0.013888889	1	0.047619048	1
0.040257112	0.716112532	0.1	0.998721228	0.036537468	0.760869565	0.026403718	0.791954745	0.020187793	0.789440603	0.013888889	1	0.047619048	1
0.041272369	0.722506394	0.1	0.998721228	0.037169023	0.767263427	0.026649149	0.801382778	0.020500522	0.795725959	0.013888889	1	0.047619048	1
0.041293666	0.728900256	0.1	0.998721228	0.037726098	0.773657289	0.02690618	0.808925204	0.020687872	0.802639849	0.013888889	1	0.047619048	1
0.041951745	0.735294118	0.1	0.998721228	0.038645132	0.781329923	0.027452191	0.817724701	0.020938897	0.808925204	0.013888889	1	0.047619048	1
0.042489476	0.74168798	0.1	0.998721228	0.038823644	0.789002558	0.028009693	0.82212445	0.021428848	0.815210559	0.013888889	1	0.047619048	1
0.043167796	0.748081841	0.1	0.998721228	0.039360529	0.796675192	0.028303418	0.832181018	0.021724334	0.821495915	0.013888889	1	0.047619048	1
0.043767559	0.754475703	0.1	0.998721228	0.040342845	0.803069054	0.028811505	0.840980515	0.022108774	0.828409805	0.013888889	1	0.047619048	1
0.04411368	0.760869565	0.1	0.998721228	0.041225455	0.810741688	0.029767196	0.848522942	0.0224497	0.835952231	0.013888889	1	0.047619048	1
0.044232906	0.767263427	0.1	0.998721228	0.041960837	0.81713555	0.030043759	0.856065368	0.022987229	0.842237586	0.013888889	1	0.047619048	1
0.044444432	0.773657289	0.1	0.998721228	0.042231621	0.823529412	0.030670132	0.863607794	0.02331244	0.848522942	0.013888889	1	0.047619048	1
0.044730115	0.780051151	0.1	0.998721228	0.042955129	0.829923274	0.031733661	0.87115022	0.023845007	0.856693903	0.013888889	1	0.047619048	1
0.045099843	0.786445013	0.1	0.998721228	0.043552337	0.836317136	0.032742707	0.878692646	0.024143351	0.864236329	0.013888889	1	0.047619048	1
0.045256776	0.792838875	0.1	0.998721228	0.044082687	0.842710997	0.032985386	0.884978001	0.024509804	0.871778755	0.013888889	1	0.047619048	1
0.045687346	0.799232737	0.1	0.998721228	0.045043126	0.849104859	0.033552436	0.891263356	0.024807136	0.878064111	0.013888889	1	0.047619048	1
0.04615634	0.805626598	0.1	0.998721228	0.045529716	0.856777494	0.034029704	0.897548712	0.02518083	0.884349466	0.013888889	1	0.047619048	1
0.046428592	0.81202046	0.1	0.998721228	0.046071749	0.863171355	0.03441581	0.904462602	0.025803036	0.890634821	0.013888889	1	0.047619048	1
0.04674454	0.818414322	0.1	0.998721228	0.04706634	0.869565217	0.034794309	0.910747957	0.026056338	0.896920176	0.013888889	1	0.047619048	1
0.048532366	0.824808184	0.1	0.998721228	0.049453162	0.875959079	0.035566341	0.916404777	0.026983027	0.903834067	0.013888889	1	0.047619048	1
0.049999998	0.831202046	0.1	0.998721228	0.050807559	0.884910486	0.036470558	0.922690132	0.027982861	0.910119422	0.013888889	1	0.047619048	1
0.05	0.837595908	0.1	0.998721228	0.052390623	0.891304348	0.037213526	0.928975487	0.028642481	0.916404777	0.013888889	1	0.047619048	1
0.05	0.84398977	0.1	0.998721228	0.052988752	0.89769821	0.03833149	0.935260842	0.030551416	0.922690132	0.013888889	1	0.047619048	1
0.052419856	0.850383632	0.1	0.998721228	0.055667664	0.906649616	0.039662863	0.942803268	0.032452713	0.928975487	0.013888889	1	0.047619048	1
0.056774394	0.856777494	0.1	0.998721228	0.057400965	0.914322251	0.040461192	0.947831552	0.033074479	0.937146449	0.013888889	1	0.047619048	1
0.06062302	0.863171355	0.1	0.998721228	0.061395349	0.923273657	0.041597937	0.954116908	0.033759023	0.943431804	0.013888889	1	0.047619048	1
0.065588326	0.869565217	0.1	0.998721228	0.064048525	0.933503836	0.044087514	0.959773727	0.034542385	0.949717159	0.013888889	1	0.047619048	1
0.068396609	0.875959079	0.1	0.998721228	0.066363976	0.941176471	0.044756918	0.965430547	0.035465484	0.956002514	0.013888889	1	0.047619048	1
0.069527984	0.882352941	0.1	0.998721228	0.068679981	0.950127877	0.048211857	0.96920176	0.037357316	0.962287869	0.013888889	1	0.047619048	1
0.071065031	0.89258312	0.1	0.998721228	0.070071672	0.959079284	0.05533779	0.972972973	0.03846401	0.968573224	0.013888889	1	0.047619048	1
0.07450421	0.900255754	0.1	0.998721228	0.074834991	0.968030691	0.060460199	0.976115651	0.039683586	0.97485858	0.013888889	1	0.047619048	1
0.077114693	0.906649616	0.1	0.998721228	0.078689202	0.976982097	0.062197449	0.979258328	0.041335584	0.981143935	0.013888889	1	0.047619048	1
0.079280672	0.914322251	0.1	0.998721228	0.084417494	0.988491049	0.065406531	0.982401006	0.049444119	0.988686361	0.013888889	1	0.047619048	1
0.080697865	0.920716113	0.1	0.998721228	0.092175644	0.997442455	0.066994396	0.985543683	0.054755784	0.995600251	0.013888889	1	0.047619048	1
0.081408161	0.927109974	0.1	0.998721228	0.092175644	0.997442455	0.071350968	0.988686361	0.054755784	0.995600251	0.013888889	1	0.047619048	1
0.08344585	0.938618926	0.1	0.998721228	0.092175644	0.997442455	0.075552489	0.991829038	0.054755784	0.995600251	0.013888889	1	0.047619048	1
0.086323147	0.945012788	0.1	0.998721228	0.092175644	0.997442455	0.079391738	0.994971716	0.054755784	0.995600251	0.013888889	1	0.047619048	1
0.087690757	0.955242967	0.1	0.998721228	0.092175644	0.997442455	0.090465105	0.998114393	0.054755784	0.995600251	0.013888889	1	0.047619048	1
0.088465813	0.962915601	0.1	0.998721228	0.092175644	0.997442455	0.090465105	0.998114393	0.054755784	0.995600251	0.013888889	1	0.047619048	1
0.090000018	0.974424552	0.1	0.998721228	0.092175644	0.997442455	0.090465105	0.998114393	0.054755784	0.995600251	0.013888889	1	0.047619048	1
0.09348908	0.982097187	0.1	0.998721228	0.092175644	0.997442455	0.090465105	0.998114393	0.054755784	0.995600251	0.013888889	1	0.047619048	1
0.1	0.993606138	0.1	0.998721228	0.092175644	0.997442455	0.090465105	0.998114393	0.054755784	0.995600251	0.013888889	1	0.047619048	1

==> ISIT_reviews.tex <==
\section*{Comments from ISIT reviewers and basic thoughts on how to address them}
\textcolor{blue}{
\begin{enumerate}
    \item While the paper describes a clear optimization problem, it does not attempt to propose any upper or lower bounds on the achievable rate (or proportional fair throughput) that can be efficiently evaluated for a given configuration.
    \begin{itemize}
        \item We will do new simulations with resource reuse, as discussed in the meeting. We will also make the call to the lower bound bolder.
        \item Kagan will do a new simulation: Fixed L (as changing L will result in non-integer t), multi-round delivery, freq. reuse factor of 3 (interference-free). We will also put a step CDF for the ultimate optimum case: fixed and known U.
    \end{itemize}
    \item It is also good practice to compare the performance of a proposed algorithm to other known approaches in the literature. In this case, one could have evaluated the performance of other caching solutions or "naive" solutions that ignore the possibility of caching.
    \begin{itemize}
        \item There is no other comparable scheme. But we have to clarify that the L=1 case is really how trivial CSMA networks are simulated nowadays.
    \end{itemize}
    \item When highlighting the keyword ‘fairness’, the authors have not explained the intuition and physical meaning of fairness. The optimization problem (4) is not well motivated, and the parameter to be optimized ‘a’ is not defined.
    \begin{itemize}
        \item Giuseppe will add some text to make it clear that the convex haul is achievable...
    \end{itemize}
    \item There are many unclear assumptions and statements. For instance, the authors mentioned in the introduction and abstract about handling sequential requests for consecutive chunks, however, this assumption has not been mentioned in the caching design part and optimization part. Also, it is claimed in the beginning that the rate needs to be higher than the streaming rate. This is also not mentioned in the technical part.
    \item The system model seems to be less practical or has not been explained clearly. The condition for a user to be served without interference seems to be strict. In Fig1, two of the users will not be served. And how will different values of the radiuses affect the proposed method?
    \item The authors are suggested introducing the cache condition at helpers and servers and also clarifying the roles they play respectively. How about the content delivery phase between helper and server?
    \item How is this work compared with [11]? The proposed method seems like a simple extension of the cache replication scheme in [11] by considering multi-helpers that can be inactive. However, the helper activation is assumed to be given in an exhaustive manner. Hence the cache policy is not dependent on the activation that much. It makes more sense if probabilistic activation is considered utilizing the statistics of helper inactivity.
    \item  More explanation of the upper bound given in (3) needs to be given. It is unclear to me how it is derived from (2).
    \begin{itemize}
        \item Stupid comments in items 4-8, overall. But we can try to make the text better to avoid similar confusion.
    \end{itemize}
    \item Some typos Page2, the notation of codeword is not consistent, $c_j$,  $S_j$…. Page 3 IIIA, I(i) extra the number.
    \begin{itemize}
        \item We have to check these carefully.
    \end{itemize}
    \item  I cannot fully understand the main difference between [7] and this paper, regarding the single-request assumption of [7] (which is not compatible with the real-world implementation of CC form the perspective of authors) and sequential request for the chunks of a specific video file. As I know, in most of the state-of-the-art papers in this field of study, a video file is requested by one of the users and server transmits some coded messages to fulfill its demand. There is no need for requesting the chunks of a specific video file.
    \item As far as I know, in decentralized cache placement, each user stores a subset of files uniformly at random and independent of other users but I fail to find out the concept of the decentralized cache placement in the paper. Please clarify the decentralized cache placement using the cache profiles.
    \item In system model, you mentioned that there exist a total number of N chunks for all video files. Nonetheless, in the next paragraph, each video file has been split into t choose L sub-packets. Do you mean that there is a library of N distinct video files with the size of F bits?
    \begin{itemize}
        \item Comments 10-12 are easy to address with more explanation in the text.
    \end{itemize}
    \item It is a bit difficult to follow the defined parameters, perhaps it would be better to put a table into the appendix to summarize the defined parameters.
    \item Perhaps, I misunderstood the definitions but are there typos in Example 1 while creating preliminary codewords because according to the definition in (1), shouldn’t we have $W_{d3,{1}}$ and $W{d_4,{2}}$? If this is the case, the same typo exists in Example 2 as well.
    \item It will be better to have a more detailed discussion on the comparison of the two heuristic approaches so that we can understand the trade-off that each technique creates.
    \item It will be insightful to have a discussion on the potential future directions.
    \begin{itemize}
        \item Again, easy items to address... I really wonder why this paper is reject with such loose comments :(
    \end{itemize}
\end{enumerate}
}

==> Intro.tex <==
%\todo[inline]{bold-face sentences to be checked by Kagan}

The increasing amount of data traffic, especially driven by multimedia applications, has necessitated the development of new communication techniques. One interesting resource is on-device memory; it is cheap and can be used to proactively store a large part of multimedia content, e.g., for video-on-demand (VoD) applications. As a result, many researchers have considered the efficient use of onboard memory in the context of \emph{caching}. Pioneering works in this regard introduced femtocaching~\cite{shanmugam2013femtocaching} and F-RAN models~\cite{park2016joint}. A major breakthrough happened with the introduction of coded caching (CC)~\cite{maddah2014fundamental}, which showed that a speedup factor in the achievable rate, scaling with the cumulative cache size in the network, is possible by multicasting carefully created codewords. Later, many works extended the original work of~\cite{maddah2014fundamental}, e.g., for wireless~\cite{tolli2017multi}, multi-server~\cite{shariatpanahi2016multi}, multi-antenna~\cite{shariatpanahi2018physical}, and multi-hop networks with helpers assisting the communication~\cite{mozhgan}. 
%Many extensions of the original model exist, e.g., for wireless links~\cite{tolli2017multi}, multi-server~\cite{shariatpanahi2016multi} and multi-antenna~\cite{shariatpanahi2018multi,salehi2021MIMO} setups, and multi-hop networks with or without processing capabilities in the middle nodes~\cite{mozhgan}. 
Meantime, many challenges hindering the applicability of CC techniques in real networks were addressed. For example, the subpacketization bottleneck was studied for single- and multi-antenna setups~\cite{lampiris2018adding,salehi2020lowcomplexity}, simpler beamformer designs were introduced~\cite{salehi2020lowcomplexity,mahmoodi2021low}, and the problem of supporting network dynamicity was addressed~\cite{caire,salehi2021low,abolpour2022coded}.

In this paper, following a system model similar to~\cite{mozhgan}, we consider the application of CC in two-hop wireless local area networks (WLAN), where a single server transmits data to a large number of users through multiple access points (AP). WLANs play an important role in wireless data delivery; they facilitate data access, e.g., in our homes, malls, airports, and cars. Two important properties of WLANs are a) unit frequency reuse due to the scarce availability of unlicensed bands and b) the collision-type interference model (i.e., packets are lost if a receiver gets the superposition of concurrent packets, all above a certain interference threshold, from different APs). Considering multi-AP WLANs and single per-user requests, the authors in~\cite{mozhgan} optimized the worst-case delivery time of all requests. Using basic principles of the multi-round delivery method in~\cite{caire} (which was later proved by~\cite{parinello} to be optimal for the shared-cache model), they first used graph coloring to construct a reuse pattern of APs and optimized the AP-user allocation to minimize the delivery time. Next, they introduced the `Avalanche' algorithm to leverage the interference-free state of the users as APs finished their multi-round delivery.

%This paper builds upon earlier work in~\cite{mozhgan} on extending the original scheme of~\cite{maddah2014fundamental} to two-hop networks. We use the same data placement and user allocation to caching profiles as in~\cite{caire} as it allows handling network dynamicity with controlled subpacketization. We build our work upon the more practical broadcast/collision model used there, which considers a network with broadcast constraints at the helpers and collision interference at the users. The work in~\cite{mozhgan} considers the case where each user in the system requests a single file and investigates the worst case delivery time of all of the user requests. 
%Based on multi-round delivery of ~\cite{caire}, which was proven to be optimal for the shared-link model in \cite{parinello}, Mozhgan et. al. use graph coloring for constructing a reuse pattern of helpers and then optimize the allocation between the helpers and the users and also another method which they call Avalanche where they leverage users becoming free of interference when helpers finish their multi-round delivery. 
Both the graph coloring and avalanche schemes of~\cite{mozhgan} are heuristic methods, however, and while they compare well with the multi-round method of~\cite{caire}, neither of them achieves any optimality metric. Moreover, the single-request assumption of~\cite{mozhgan} is not appealing for real-world implementation of CC techniques in WLAN. This is because, in practice, CC applied to VoD streaming requires the sequential delivery of a long sequence of ``chunks’’ forming the streaming session. Each chunk contains a relatively small segment of video, and the chunks must be delivered at a rate (slightly) higher than the playback rate at which the video buffer is emptied at the user video player application.  Hence, the most important requirement is the delivery rate in terms of chunks per unit of time rather than the worst-case single-request delivery time considered by~\cite{mozhgan}. Accordingly, in this paper, we consider a multi-AP WLAN model similar to~\cite{mozhgan} but with sequential requests. We obtain a computational way to determine the theoretical throughput region of per-user delivery rates and solve the fairness scheduling problem, which maximizes a desired fairness metric of user delivery rates over this region. We also provide two heuristic methods based on restricting the throughput region and a greedy algorithmic approach to achieve a sub-optimal solution with reduced complexity. Numerical analyses are used to evaluate the performance of the proposed solutions.

%(Maybe no need to mention this:The problem in Avalanche lies in the fact that for initialization it assumes that there are users which are in the tranmission radius of a helper free from interference of other helpers and also while the algorithm is running if more than one helper finish at the same time there may not be another helper to serve the users which are freed from their interference since they may be the only ones who can serve them at the first place.)

%(\textbf{WRITE THE MAIN CONTRIBUTIONS OF MOZHGAN'S WORK}, we formulate the problem as \textcolor{blue}{designing a transmission strategy over a set of possible actions, and show that the problem can be solved with linear programming (?). However, the complexity grows exponentially (?) with network dimensions. Then, we introduce a heurisitic algorithm to solve the problem sub-optimally. Finally, we show through simulations that the gap between the heurisitic method and the optimal solution is small.} \textbf{WRITE YOUR OWN IDEA OF OUR CONTRIBUTION INSTEAD OF THE BLUE TEXT.})

%\todo[inline]{the super-user idea should be fit in-between}

%\todo[inline]{I need to read Mozhgan's paper and talk with Kagan to find the novelty aspects better}

%\todo[inline]{Should we go into details of the video delivery application already in the introduction? If we have extra space, we will put one paragraph here.}

%\todo[inline]{One paragraph describing the notations. Mohammad will do that.}
%So, $\Ba$ is a vector, and $\BA$ is a matrix, and $\CA$ is a set.

%In this paper, we have used the following notations...
We have used boldface lower- and upper-case letters to denote vectors and matrices, respectively. Sets are represented by calligraphic letters. $\Bv[i]$ is the element $i$ of vector $\Bv$, and $\CA \backslash \CB$ denotes the set of elements of $\CA$ not in $\CB$. For integer $J$, $[J]$ represents the set $\{1,2,\cdots,J\}$. $\binom{n}{k}$ denotes binomial coefficient, and its value is zero if $n < k$. %Other notations are defined as used in the text.

%\todo[inline]{Here starts the revised text}



%The intro and abstract will take about 1 page.


%In the introduction:
%\begin{enumerate}
%    \item Why we are doing this? There is lots of traffic ...
%    \item CC scheme is good to address this issue ...
%    \item There are problems and some of them are addressed ...
%    \item One other issue is the application of CC techniques in a multi-level network. In this paper, we address the ...
%    \item Some other ideas: users are repeatedly asking for content, and references to the previous work, ...
%    \item A paragraph briefly explaining the idea and novel parts. Novel parts are the original solution, the super-user idea and the algorithm.
%    \item A paragraph or sentence about how you are evaluating your new algorithm and what are the results.
%\end{enumerate}

%Some other notes:
%\begin{enumerate}
%    \item We need to explain the super-user idea already in this paper. Because otherwise, we cannot produce nice simulation results.
%\end{enumerate}

==> SysModel.tex <==
%The system model will take about 0.75 of a page.

%Put figures for the system model and the graphs.

%Explain the caching scheme.

%Explain the problem, which is how to do the delivery.

%You can briefly discuss the next chapters: we first solve the problem using solutions with convex optimization (Analytical solutions), and then, provide a heuristic solution (Put a name for your algorithm).

%\textbf{WRITE THE SYSTEM MODEL BEFORE GOING INTO THE TECHNICAL DISCUSSIONS.} \\

%\todo[inline]{here starts the text:}

\begin{figure}[t]
    %\begin{subfigure}{0.3\columnwidth}
        \centering
        \includegraphics[width = 0.8\columnwidth]{Figs/NetworkModel.png} %\label{fig:network_model}
        \vspace{-1pt}
    \caption{Example network with $H=2$, $K=5$.}
    \vspace{-12pt}
    \label{fig:network_model}
\end{figure}


The system model considered in the paper is similar to the broadcast/collision model of~\cite{mozhgan}: a single server, connected to $H$ helper nodes (APs in WLAN) via error-free fronthaul links,
%of capacity $C_{\mathrm{front}}$, 
serves the requests of $K$ cache-enabled users. We use $h_i$ and $u_k$, $i \in [H]$ and $k \in [K]$, to represent helpers and users, respectively. Every $u_k$ is connected to a limited number of helpers via a wireless access network, and every $h_i$ has 
%a multicast capacity of $C_{\mathrm{access}}$, 
an effective transmission radius of $r_{\mathrm{trans}}$ and an interference radius of $r_{\mathrm{inter}} \ge r_{\mathrm{trans}}$. We call a helper $h_i$ `active' at a time instant if it is transmitting data in that time instant. Denoting the locations of the helper $h_i$ and user $u_k$ as $\Sfx(h_i), \Sfx(u_k) \in \mathbb{R}^2$, respectively, $u_k$ can successfully decode the transmitted message of $h_i$ if and only if 1) $|\Sfx(h_i) - \Sfx(u_k)| \le r_{\mathrm{trans}}$, and 2) there is no other active helper node $h_{i'}$ such that $|\Sfx(h_{i'}) - \Sfx(u_k)| \le r_{\mathrm{inter}}$. A graphical representation of the system model is shown in Figure~\ref{fig:network_model}.

In this paper, we consider a video streaming application as the use case. We assume every video file is split into multiple `chunks' each representing a few seconds of the multimedia content. A user streaming a video generates a sequence of requests for the corresponding chunks of that video. Let us assume there exist a total number of $N$ chunks (for all video files), every chunk has the same size, and every user has a cache memory large enough to store at most $M<N$ chunks. Let us also use $W_n$, $n \in [N]$, to denote a general video chunk.% and $\CF$ to represent the set of all chunks. 

%The total multicast capacity of each helper is assumed to be $C_{\mathrm{access}}$.

%We have the broadcast/collision model of \cite{mozhgan} where we have one server, $H$ helpers, $N$ files $W_n$ where $n\in{\lbrace1,2,...,N\rbrace}$ and each file $W_n$ has $F$ bits and $K$ users where each user can cache up to $MF$ bits and $M\in{\lbrace0,1,...,N\rbrace}$. The server is connected to the helpers with $H$ error-free fronthaul links with capacity $C_{front}$ bits/s where each helper has a multicast capacity of $C_{access}$ bits/s. Each helper $h_i$ and each user $u_k$, where $i\in{\lbrace1,2,...,H\rbrace}$ and $k\in{\lbrace1,2,...,K\rbrace}$, are on a 2-dimensional plane in $\mathbb{R}^2$ such that the positions of user $u_k$ and helper $h_i$ on the plane will be denoted by $x(u_k)$ and $x(h_i)$ respectively where $x(h_i),x(u_k)\in{}\mathbb{R}^2$. Each helper $h_i$ has a radius of effective transmission $r_{trans}$ and a radius of interference $r_{inter}$ such that $r_{trans}\leq{}r_{inter}$. A  user $u_k$ can successfully decode the transmitted message of $h_i$ if and only if $\vert{}x(h_i)-x(u_k)\vert{}\leq{}r_{trans}$ and there is no other helper $h_{i'}$ transmitting a message at the same time instance where $\vert{}x(h_{i'})-x(u_k)\vert{}\leq{}r_{inter}$. We say that a helper $h_i$ is `active' at a time instance if it is transmitting.

System operation consists of two phases, placement, and delivery. During the placement phase, users' cache memories are filled up with subpackets (i.e., smaller portions) of all the video chunks. Due to its low subpacketization overhead, we use the decentralized cache replication algorithm of~\cite{caire,parinello}. With this model, instead of defining cache contents for every user individually, we fix a number of $L < K$ \emph{cache profiles} and assign each user randomly to one of the profiles. Let us use $\SfL(u_k) \in [L]$ to denote the cache profile assigned with user $u_k$. Given $L$, we define $t = \frac{LM}{N}$ and divide every chunk $W_n$, $n \in [N]$, into $\binom{L}{t}$ non-overlapping equal-sized subpackets $W_{n,\CS}$, where $\CS$ can be any subset of $[L]$ with size $|\CS| = t$. Then, if $\SfL(u_k) = l$ for a user $u_k$, it stores every subpacket $W_{n,\CS}$, for every $n \in [N]$ and $\CS \ni l$. Clearly, using this algorithm, all users assigned to the same profile cache the same data.

%For the cache placement, we use the decentralized cache replication method of \cite{caire} which is an extension of the MAN cache placement \cite{maddah2014fundamental}. We fix $L<K$ and define $\gamma=LM/N$ where $\gamma$ is an integer and $0\leq{}\gamma\leq{}L$, and we divide every file $W_n$ to $\binom{L}{\gamma}$ non-overlapping equal sized subfiles  $W_{n,\mathcal{T}}$ where $\mathcal{T}\in{\Omega_\gamma^L}$ such that $\Omega_\gamma^L=\lbrace{}U\subseteq{\lbrace1,2,...,L\rbrace} : |U|=\gamma\rbrace{}$. For each user $u_k$, where $k\in{\lbrace1,2,...,K\rbrace}$, an integer $l\in{\lbrace1,2,...,L\rbrace}$ is randomly chosen independently of the other users which corresponds to the cache group of the user and user $u_k$ caches the subfiles $W_{n,\mathcal{T}}$ for all  $\mathcal{T}\ni{l}$ and all $n\in{\lbrace1,2,...,N\rbrace}$. Notice that the subfiles stored in the caches of the users in the same cache group are identical.

During the delivery phase, users reveal their requested video chunks (corresponding to the videos they want to stream). We assume users can start streaming at arbitrary times. However, when they start streaming, they repeatedly generate requests for consecutive video chunks; i.e., after receiving every single chunk, each user immediately generates a new request for the subsequent chunk. With this model, we can safely assume a single chunk is requested by at most one user at a given time, as even if two users are streaming the same video, it is unlikely that they have started streaming at the same time. Given the set of user requests and
%In this paper, we consider data delivery after every user has revealed their requested chunk sequence. Then, 
using a delivery algorithm, 
the server creates a number of codewords and transmits each codeword to a subset of users through a selection of active helpers. The goal is to serve requested video chunks while optimizing a performance function of, e.g., delivery time, energy, or fairness.

%In this paper, we first use the following two simplifying assumptions to find an optimal delivery solution in Section~\ref{section:optimal_solution}: 1) network topology is static, and the users do not move during the delivery session, and 2) each user instantly requests another file after it receives the previously requested one.\footnote{A real-world example can be a video delivery application in a large hall (e.g., an airport), where multiple Wi-Fi routers facilitate data transmission. Files in $\CF$ represent chunks of the video files, and every user requests the next chunk right after it finishes the reception of the previous one.}
%We also assume the worst-case scenario where the users request different files.\footnote{This is a fair assumption for the example video delivery application. This is because even if two users are watching the same video, there is little chance that they have started streaming simultaneously.}
%Then, in Section~\ref{section:kagan_solution}, we provide a heuristic solution that supports dynamic network conditions and non-continuous file requests.

%\todo[inline]{the following part needs changing: users are static and always have requests. there is no concept of a time frame}
%In this paper, we slightly simplify this model: we assume the time horizon is divided into multiple time frames, and users' requests are queued until the starting point of the next frame. Then, at the beginning of each frame, the server fetches every request in the queue and uses the delivery algorithm to serve them efficiently. We assume users being served in a time frame do not change their locations during that frame. The next time frame begins right after all the requests at the beginning of the previous frame are fully served. Using this model, without losing practicality, we can assume the same procedure is repeated in each frame and eliminate the frame index.

With $H$ helpers that can be either active or inactive, there exist $2^H$ selections for the \emph{activation pattern} of the helpers. Let us use vectors $\Bp_j$, $j \in [2^H]$, to denote activation patterns. Every $\Bp_j$ has $H$ binary elements $\Bp_j[i]$, $i \in [H]$, and $\Bp_j[i] = 1$ only if helper $h_i$ is active in the corresponding activation pattern. The activation pattern determines which users can be served by each active helper and whether they can be served by multicasting codewords instead of unicasting.
%the user(s) that each active helper can serve. It also clarifies if these users can be served through codeword multicasting:
Following the cache placement phase, 
a codeword can be created for every subset of users $\CV$ of size $0 < |\CV| \le t + 1$ if all users in $|\CV|$ are served by the same active helper $h_i$ but have distinct cache profiles. Of course, due to the repetition in cache profile assignments and multiple choices for the size of $\CV$, there may exist multiple codeword creation possibilities for each helper.
Codeword creation follows the same basics of~\cite{maddah2014fundamental,caire} and is explained in more detail in Section~\ref{section:optimal_solution}. %Multicasting enables more users to be served with a single transmission, thus enhancing the system's performance. 
%So, intuitively, we like to create as many codewords as possible for any given activation pattern $\Bp_j$.




%A coded transmission through active helper $h_i$ is possible if the users served by $h_i$ are assigned to different cache profiles.
%
%Given a pattern $\Bp_j$, the server may be able to create one or multiple codewords for every active helper $h_i$.
%The final step is determining which users could be served simultaneously with a single codeword. 
 
%(i.e., $\SfL(u_k) \neq \SfL(u_m)$ for distinct users $u_k, u_m \in \CU_i$). 

%\todo[inline]{we should provide a hint to how the codewords are created, either in general form or using an example}
%Of course, here we have the extra condition that the users served by a single codeword should all be connected to (\textbf{DEFINE CONNECTION}) the same helper node.
%\todo[inline]{Maybe an example here.}

The server may need to choose multiple activation patterns to serve all the requests. This is because it is likely that for a specific pattern $\Bp_j$, some users could not be served at all due to interference from active helpers. 
%Multiple patterns may be activated over various communication resources. In this paper, we assume consecutive time slots are used, where every pattern $\Bp_j$ is activated for $a_j \ge 0$ seconds. 
Moreover, as discussed, we may have multiple choices for codeword creation with every activation pattern. Let us assume the number of such choices for activation pattern $\Bp_j$ is $\Sfc(\Bp_j)$.
We use the term \emph{policy} to refer to a selection of an activation pattern and a codeword creation choice, and $\pi(j,s_j)$ to represent the policy resulting from activation pattern $\Bp_j$ and codeword choice $s_j$, $s_j \in [\Sfc(\Bp_j)]$. 
Clearly, the total number of policies is $\sum_{j \in [2^H]} \Sfc(\Bp_j)$.
Every policy $\pi(j,c_j)$ results in a rate vector $\Br(j,c_j)$, where the element $k$, $k \in [K]$, in $\Br(j,s_j)$ denotes the rate of user~$u_k$ with policy $\pi(j,s_j)$. The network throughput region is defined as the convex hull of all rate vectors, shown by $\mathrm{Conv}(\Br(j,s_j))$. The goal is to optimize a fairness function of the rate values, which can be any concave component-wise non-descending function over $\mathrm{Conv}(\Br(j,s_j))$. For example, we may choose any function from the alpha-fairness family~\cite{fairness}: for $\alpha = 1$, we get proportional fairness; for $\alpha = 0$, we get sum-rate (unfair); and for $\alpha \rightarrow \infty$, we get max-min (hard) fairness. In this paper, for the sake of brevity, we chose the proportional fairness function $\Sff = \sum_k \log(r_k)$ as our metric, where $r_k$ is the time-averaged delivery rate of user ~$u_k$ (usually referred to as the `throughput rate’).

%Successful data delivery may require using multiple policies, which can be done over various communication resources. In this paper, without loss of generality, we assume consecutive time slots are used, where every policy $\pi(j,s_j)$ is used for $a(j,s_j) \ge 0$ seconds. 
%As we will see in Section~\ref{section:optimal_solution}, every policy $\pi(j,s_j)$ results in a rate vector $\Br(j,s_j)$, where the element $k$, $k \in [K]$, in $\Br(j,s_j)$ denotes the rate of user~$u_k$ with policy $\pi(j,s_j)$. Then, the sum rate vector can be defined as
%\begin{equation}
%    \Br_{\mathrm{sum}} = \sum_{j \in [2^H]} \sum_{s_j \in [\Sfc(\Bp_j)]} a(j,s_j) \Br(j,s_j) .
%\end{equation}
%Let us denote the sum rate of user~$u_k$ (i.e., the element $k$ of $\Br_{\mathrm{sum}}$) as $r_k$.  
%In this paper, we use the proportional fairness function $\Sff = \sum_k \log(r_k)$ as our metric\footnote{In fact, we can choose any function from the alpha-fairness family: for $\alpha = 1$ we get proportional fairness, for $\alpha = 0$ we get sum-rate (unfair), and for $\alpha \rightarrow \infty$ we get max-min (the hard fairness). In this paper, proportional fairness is chosen for sake of brevity.} and try finding $a(j,s_j)$ values such that $\Sff$ is maximized.\\



% \begin{figure}[t]
%     \centering
%     \begin{tikzpicture}[scale=0.6,transform shape]

%         \draw[thick] (2,2) circle (2 cm);
%         \draw[thick] (5,2) circle (2 cm);
%         \draw[red!50,fill=red!50](2,2) circle (0.1 cm);
%         \draw[red!50,fill=red!50](5,2) circle (0.1 cm);
%         \draw[dashed] (2,2) circle (2.7 cm);
%         \draw[dashed] (5,2) circle (2.7 cm);
%         \draw[blue!50,fill=blue!50](3.5,2) circle (0.05cm);
%         \draw[blue!50,fill=blue!50](3,3.2) circle (0.05cm);
%         \draw[blue!50,fill=blue!50](1.2,1.3) circle (0.05cm);
%         \draw[blue!50,fill=blue!50](5.5,2.9) circle (0.05cm);
%         \draw[blue!50,fill=blue!50](4.8,0.8) circle (0.05cm);

%     \end{tikzpicture}
%     \caption{Example network with $H=2$, $K=5$.}
%     \label{fig:network_model}
% \end{figure}

%In this example number in parantheses corresponds to cache group $l$ of the users. $L=3$, $\gamma=1$. We have $3$ instantaneous maximal rate vectors which maximizes the number of users per helper and 3 maximal superuser vectors. $[0.5, 0, 0, 0, 0.33, 0.33]$, $[0.33, 0.33, 0.33, 0, 0]$ and $[0, 0, 0.33, 0.33, 0]$ corresponds to former, $[0.5 ,0 ,0 ,0 ,0.33, 0.33]$, $[0.33 ,0.33 ,0.33 ,0 ,0]$ and $[0, 0 ,0.167 ,0.33 ,0.167]$ corresponds to latter.


%As we will see in Section~\ref{section:optimal_solution}, a selection of an activation pattern and a codeword creation choice results in a rate vector $\Br_q$, $q \in Q$, where $Q = \sum_{j \in [2^H]} \Sfc(\Bp_j)$ is the total number of such selections and the element $k$, $k \in [K]$ in $\Br_q$ denotes the rate of user $u_k$ if policy $\pi_q$ is selected. 

%\todo[inline]{here comes the definition of the rate}

%Moreover, for a given activation pattern of helpers, the server may have multiple choices for creating codewords (as multiple users with the same cache profile may be connected to the same active helper). The result is multiple rate vectors $\Br$ ...

%Also, the server may have to choose multiple activation patterns in a single time frame, as every user requesting data at the beginning of the time frame may not be served with a single activation pattern. Multiple activation patterns could be activated over any orthogonal network resource. In this paper, we assume the time frame is split into smaller time intervals of size $a_j$, and the rate vector $\Br_j$ is achieved for a time duration of $a_j$. The goal is to find out the rate vectors $\Br_j$ and the weights $a_i$ such that ...
%\todo[inline]{The optimization problem comes here.}
%\todo[inline]{Big question: where to discuss how the rate vectors are created?}

%\todo[inline]{The discussion should be more general here: given a specific pattern, the server has multiple choices for creating codewords, depending on which users could be served by every active helper and what the assigned profile of each user is. The selection of active helpers and the users to be served provides us with a respective rate vector for that activation pattern. The goal is to describe how this vector could be found, then. The question is, where to describe each part? System model or the next section?}
%\todo[inline]{I think it is better to describe the codeword generation process here, maybe a toy example. The graph representation can be moved to the next section, then. But the rate function should be defined here.}
%consider a set of users $\CU_h$ that all can receive data from an active helper $h \in [H]$ and every user $u_k \in \CU_h$ is assigned to a different cache profile $\SfL(k) \in [L]$. As the number of profiles is $L$, we must have $|\CU_h| \le L$. Then, for every non-empty subset of users $\CT_h \subseteq \CU_h$ with $|\CT_h| \le \gamma+1$, the server can create the codeword
%\begin{equation}
%\label{eq:exmp_XOR}
%    \bigoplus_{u_k \in \CT_h} W_{d_k,} \quad,
%\end{equation}
%where $\oplus$ denotes the bit-wise XOR operation, and send it to every user $u_k \in \CT_h$ through helper $h$, so that every user $k \in \CT_h$ receives part of its requested file $W_{d_k}$. This is possible because after receiving the codeword, every user $u_k \in \CT_h$ can use its cached content to remove the unwanted terms, and decode ... .

%\todo[inline]{now we should explain the delivery phase. Mohammad to do this by 27.1}

%During the delivery phase, network users reveal their requested files.
%\begin{itemize}
%    \item multiple codewords can be sent in parallel.
%    \item we have many choices for activation patterns.
%    \item we need to have multiple time intervals to serve all the users (as all the users might not be served with a single pattern).
%    \item every selection of activation pattern gives us a rate vector.
%    \item the length of the time intervals should also be defined.
%    \item the goal is to optimize the $\sum \log$ function.
%\end{itemize}

%\todo[inline]{The old text}

%As in \cite{mozhgan}, the number of XORs a helper needs to serve all the users in its delivery column is $\binom{L}{\gamma+1}-\binom{L-l'}{\gamma+1}$ where $l'$ is the number of users in the delivery column.

%(We assume $F=C_{access}=C_{front}$ so that the time it takes a helper to serve all the $l'$ users in its delivery column is $(\binom{L}{\gamma+1}-\binom{L-l'}{\gamma+1})/\binom{L}{\gamma}$.)

%\todo[inline]{The old text}

%We define the rate $R_k$ of a user $u_k$ in a delivery scheme as the (average) percentage of a file $u_k$ receive per one XOR transmission. The aim of this paper is to maximize the rates of the users by also being `fair' to the users, to be more rigorous, we do proportional fairness utility maximization of the rates. Let $\mathbf{D}$ be the set of all possible delivery schemes for a fixed topology with predetermined caches of the users. Let $\mathbf{R}=\lbrace{}R_1,R_2,...,R_k\rbrace{}$. Then $\arg(\max_{\mathbf{D}}\sum_{k}\log{R_k}):=d^*$ is the delivery scheme which maximizes the proportional fairness utility function.

%In the next sections we show how to find $d^*$ exactly by using convex optimization over a convex set, we also show an (approximation) which we call the `super-user method'. We also show a heurestics method which follows a different approach but finds a rate vector $R'$ which is fairly close to the optimal rate vector $R^*$ found by using $d^*$.


